Complete equational theories for classical and quantum Gaussian relations

We give generators and relations for the hypergraph props of Gaussian relations and positive affine Lagrangian relations. The former extends Gaussian probabilistic processes by completely-uninformative priors, and the latter extends Gaussian quantum mechanics with infinitely-squeezed states. These presentations are given by adding a generator to the presentation of real affine relations and of real affine Lagrangian relations which freely codiscards effects, as well as certain rotations. The presentation of positive affine Lagrangian relations provides a rigorous justification for many common yet informal calculations in the quantum physics literature involving infinite-squeezing. Our presentation naturally extends Menicucci et al.'s graph-theoretic representation of Gaussian quantum states with a representation for Gaussian transformations. Using this graphical calculus, we also give a graphical proof of Braunstein and Kimble's continuous-variable quantum teleportation protocol. We also interpret the LOv-calculus, a diagrammatic calculus for reasoning about passive linear-optical quantum circuits in our graphical calculus. Moreover, we show how our presentation allows for additional optical operations such as active squeezing.

==> section_gaa.tex <==
%In this section, we review the theory of affine relations, as well as their presentation.  
%
%
%\subsection{Affine relations}
%\label{subsec:linrelaffrel}
%
%Before we define affine relations, recall the following less structured notion of relation: given some fixed set \(X\), an \(X\)-relation \(R:n\to m\) is a subset of the product \(R\subseteq X^n \times X^m\).  These form a compact prop:
%
%\begin{definition}
%  \label{def:xrel}
%  Given a set \(X\), the compact prop of {\em\(X\)-relations}, \(\RX\), has:
%  \begin{itemize}
%    \item \textbf{Arrows}, relations between \(X\)-relations.
%    \item \textbf{Composition} of relations \(R:n\to m\) and \(S:m\to k\) is given by:
%    \[ S\circ R \coloneqq  \{ (x,z) \in X^{n}\times X^k \ | \ \exists y \in X^m: (x,y) \in R, (y,z) \in S  \}:n\to k \]
%    \item \textbf{Identity} on \(n\), given by the diagonal relation \(\{(x,x) \in  X^n\times X^n \}:n\to n \)
%    \item \textbf{Monoidal structure}, given by the object \(0\) and the Cartesian product:
%      \[ S\times T \coloneqq \left\{\left(\begin{bmatrix}x\\y \end{bmatrix},\begin{bmatrix}z\\w\end{bmatrix}\right)  \,\middle|\,   (x,z) \in S,  (y,w)\in T \right\} \]
%    \item \textbf{Symmetric structure} is generated by the relation: 
%      \[\sigma_{1,1}\coloneqq \left\{\left(\begin{bmatrix}x\\y \end{bmatrix},\begin{bmatrix}y\\x\end{bmatrix}\right)  \,\middle|\,  x,y\in X\right\}:2\to 2 \]
%    \item \textbf{Compact structure} is generated by the relations: \[\eta_1\coloneqq \left\{\left(\bullet,\begin{bmatrix}x\\x\end{bmatrix}\right)  \,\middle|\,  x\in X\right\}:0\to 2\quad\text{and}\quad\epsilon_1\coloneqq \left\{\left(\begin{bmatrix}x\\x\end{bmatrix}, \bullet\right)  \,\middle|\,  x\in X\right\}:2\to 0\]
%  \end{itemize}
%\end{definition}
%
%Given a function \(f:X^n\to X^m\), its graph is a relation \(\Gamma_f\coloneqq \{(x,f(x))\ |\ x\in X \}:n\to m\). This assignment of a function to its graph is functorial.
%Recall the following generalization of linear transformations.  For the rest of this article we will take \(\K\) to be an arbitrary field:
%\begin{definition}
%  Given \(n,m\in\N\), a \(\K\)-affine matrix  \((T,\vec a):n\to m\) consists a \(\K\)-linear matrix \(T:n\to m\) in addition to a vector \(\vec a \in \K^m\).
%  The prop,  \(\Aff\Mat_\K\), of affine matrices has:
%
%  \begin{itemize}
%    \item \textbf{Arrows}, affine matrices.
%    \item \textbf{Composition} of \((S,\vec a):n\to m\) and \((T,\vec b):m\to k\) is given by:
%    \[
%      (T,\vec b)\circ(S,\vec a):=(TS, T\vec a +\vec b):n\to k
%    \]
%     \item \textbf{Identity} is given by \((1_n, \vec 0):n\to n\)
%    \item \textbf{Symmetric monoidal structure} is given pointwise by the direct sum.
%  \end{itemize}
%\end{definition}
%
%
%Similarly recall the following generalization of a linear subspace:
%
%\begin{definition}
%Given \(n\in\N\), an affine subspace of \(\K^n\) is a subset
%\( \{ \vec v \in \K^n \ | \ S\vec v= \vec a  \} \subseteq \K^n\)
%for some vector \(\vec a \in \K^m \) and matrix \(S:n\to m\). 
%\end{definition}
%
%Conceptually, an affine subspace is a linear subspace without an fixed origin.
%
%\begin{definition}
%The prop \(\AR\) of {\em \(\K\)-affine relations} is the  sub-prop of  \(\RK\) whose arrows \(n\to m\) are \(\K\)-affine subspaces of the vector space \(\K^n\times\K^m \cong \K^{n}\oplus \K^m\).
%\end{definition}
%
%%This is a  category because affine subspaces are closed under relational composition, and that the diagonal subset is a affine subspace. This is a compact prop because the cup, the cap and symmetry are also affine subspaces.
%
%Each affine transformation \(T: \K^{n} \to \K^{m} \) induces an affine  transformation via its graph, so that there is an embedding of props \(\Aff\Mat_\K\to \AR\).
%
%%By construction we have \(\lR \hookrightarrow \AR \hookrightarrow \RK\). In \(\lR\) and \(\AR\), the arrows \(0 \to n\) are exactly linear and affine subspaces of \(\K^n\).  In \(\lR\) there is a unique scalar \(1_0:0\to 0\), corresponding to the linear subspace \(\K^0 \subset \K^0\). But in \(\AR\) we have two scalars, the identity and the empty affine subspace \(\emptyset\subset \K^1\).
%
%\subsection{Graphical affine algebra and its interpretation}
%In this subsection, we give a graphical presentation of the prop \(\AR\). Such a presentation was first given by Bonchi et al. \cite{gaa}. However, we use the alternative presentation of affine relations given by Booth et al. \cite{gsa}.
%
%As a matter of notation, take \(\K^*\) to be the group of invertible elements in \(\K\).
%\begin{theorem}
%  \(\AR\) is presented by the compact prop \(\GAA\) which is generated by grey spiders, \(a\)-phased spiders and \(a\)-multipliers, for all \(a\in k\):
%  \begin{align*}
%    \interp{\tikzfig{figures/AffRel/b-spider}}_{\abbrar}^{\gaa}
%      &\coloneqq
%         \left\{
%           \left(
%             \begingroup
%               \renewcommand*{\arraystretch}{.7}
%               \begin{bmatrix}
%                 a\vspace*{-.2cm}\\ \vdots \\ a
%               \end{bmatrix}
%               ,
%               \begin{bmatrix}
%                 a\vspace*{-.2cm}\\ \vdots \\ a
%               \end{bmatrix}
%             \endgroup
%           \right) \in \K^{n}\oplus \K^m
%           \ \middle|\
%           a \in \K 
%         \right\} \\
%    \interp{ \tikzfig{figures/AffRel/w-spider}}_{\abbrar}^{\gaa}
%      &\coloneqq 
%        \left\{ 
%          (\vec b, \vec c)
%          \in \K^n \oplus \K^m
%          \ \middle|\
%          \sum_{j=0}^{n-1} b_j + \sum_{k=0}^{m-1} c_k  = a 
%        \right\} \\
%    \interp{ \tikzfig{figures/AffRel/mult}}_{\abbrar}^{\gaa}
%    &\coloneqq \left\{ \left(b,ab \right) \ \middle|\ b \in \K \right\}
%  \end{align*}
%  Modulo the equations making the grey and white spiders flexsymmetric as well as the equations, for all \(a,b\in \K\) and \(c \in \K^*\):
%  \[\tikzfig{figures/AffRel/axioms}\]
%
%  With the derived generators, for all \(a\in\K\):
%  \(
%    \tikzfig{figures/AffRel/scalar-daggered}
%    \coloneqq 
%    \tikzfig{figures/AffRel/scalar-twisted}
%  \)
%
%\end{theorem}
%
%
%The notions of white and grey spiders labelled by a phase-group will occur throughout the rest of this paper in different incarnations:
%
%\begin{definition}
%\label{def:phasegroup}
%  Given a group \(\mathcal{G}=(G,+,0)\), the compact prop of {\em \(\mathcal{G}\)-labelled white spiders} presented by the following equations, for all \(a,b \in G\) in addition to flexsymmetry:
%  \[\tikzfig{figures/AffRel/labelled-w-spider-axioms}\]
%
%  Similarly, the compact prop of {\em \(\mathcal{G}\)-labelled grey spiders} presented by the following equations, for all \(a,b \in G\) in addition to flexsymmetry:
%  \[\tikzfig{figures/AffRel/labelled-b-spider-axioms}\]
%  In both cases, say that \(\mathcal{G}\) is the {\em phase group} of the white and grey spiders.
%\end{definition}
%
%Therefore, we see that the white phase group of \(\GAA\) is the additive group of \(\K\); whereas the grey phase group is the trivial group. 
%
%
%\subsection{Scalable notation for graphical affine algebra}
%\label{ssec:scalable_gaa}
%In this subsection we give scalable notations for \(\GAA\).  We now can make use of the more general notion of labelled spiders:
%
%\begin{definition}
%  Scalable spiders in \(\GAA\) are defined by induction on the colour of wire \(k\in\N\).
%  The base case is trivial.
%  The inductive step is given by:
%  \begin{equation}
%    \label{eq:GAAthickspiders}
%    \tikzfig{figures/AffRel/scaledspidef}
%  \end{equation}
%\end{definition}
%
%These scalable spiders satisfy analagous axioms as before, except now the white \([k]\)-coloured spiders are indexed by the additive group of \(\K^k\).
%As a matter of notation, for any \(n,m\in\N\) take \(\Matrices\) to be the set of \(m \times n\) matrices over \(\K\).
%\begin{definition}
%  \label{def:matrix_arrow}
%Block matrices are defined by induction on the domain and codomain.  The base case is trivial.  The inductive step is given by:
%\begin{equation}
%  \label{eq:arrow_decomposition}
%  \tikzfig{figures/AffRel/blockmatex}
%\end{equation}
%
%Therefore affine matrices \((A,\vec v):n\to m \)  is represented by:
%
%\begin{equation}
%  \label{eq:affinematrix}
%  \tikzfig{figures/AffRel/affinematex}
%\end{equation}
%\end{definition}
%
%Using this notation, the image and kernel of an affine transformations \((A,\vec v):n\to m \) are respectively given by:
%
%\cole{todo}
%%\begin{equation}
%%  \interp{\tikzfig{figures/AffRel/matarrowspace1}}_{\gaa}^{\abbrar}=\ker(A)\quad\interp{\tikzfig{figures/AffRel/matarrowspace2}}_{\gaa}^{\abbrar}=\im(A)
%%\end{equation}
%%
%%And more generally the affine subspace of solutions for \(\vec v\) in the  equation \(A\vec v=\vec w\):
%%
%%\begin{equation}
%%  \interp{\tikzfig{figures/AffRel/matarrowspace3}}_{\gaa}^{\abbrar}=\left\{\vec w \,\middle|\,  A \vec w=\vec v\right\}
%%\end{equation}

